When Evidence Conflicts: Reliability-aware Meta-review Generation

Generating coherent meta-reviews from multiple peer reviews is challenging when reviewer evidence conflicts and varies in reliability. Existing approaches typically formulate meta-review generation as a multi-document summarization task and aggregate reviewer feedback uniformly, making it difficult to determine which opinions should be prioritized under disagreement. In this paper, we study meta-review generation through reliability-aware evidence aggregation. Our framework first extracts aspect-level opinions from peer reviews and identifies conflicting evidence within each aspect. It then estimates opinion-level support and review-level quality to measure evidence reliability. Based on these signals, the framework assigns reliability-aware weights to reviewer feedback, enabling the generator to prioritize better-supported arguments while preserving diverse perspectives. Experiments demonstrate that our method consistently improves meta-review generation over strong baselines on both automatic and human evaluations, with clear gains in conflict recognition and resolution under high-conflict review scenarios. The code and implementation details are publicly available at https://github.com/Wangxz729/reliability-aware-meta-review.

==> ralated_work.tex <==
2 Related Work

In this section, we discuss large-scale information 
consolidation in abstractive summarization, and
automated sentiment summarization.
2.1 Large-Scale Information Consolidation
Natural language generation systems are expected
to not only have high-quality generations but also
have the ability to comprehend the input informa-
tion, especially for conditional text generation such
as multi-document summarization which has to in-
tegrate and aggregate information from different
source documents (Gehrmann et al., 2023). Most
work in the text summarization community only
attempts to improve the generation quality of text
summarization, such as relevance and faithfulness,
without considering the intricate generation pro-
cess (Phang et al., 2022; El-Kassas et al., 2021;
Xiao et al., 2022). For example, Li et al. (2023b)
use heterogeneous graphs to represent source docu-
ments and borrow the idea of graph compression
to train the summarization model to get improve-
ment of the generated summaries. However, it is
uncertain if these models truly possess the ability
to consolidate information from different source
documents.
2.2 Automated Sentiment Summarization
Sentiment summarization aims to summarise the
overall sentiment given a set of documents (Hos-
sain et al., 2023). However, most datasets for sen-
timent summarization are in the product review
domain (Amplayo et al., 2021), and scientific sen-
timent summarization is under-explored. Meta-
review generation, which is a typical scenario of
scientific sentiment summarization, is to automati-
cally generate meta-reviews based on reviews and
the multi-turn discussions between reviewers and
the author of the corresponding manuscript (Li
et al., 2023a). It is mostly modelled as an end-
to-end task (Bhatia et al., 2020; Wu et al., 2022;
Shen et al., 2022; Chan et al., 2020). Although Li
et al. (2023a)considered the conversational struc-
ture of reviews and discussions, their models do not
explain how human meta-reviewers write the meta-
reviews. Different from investigating checklist-
guided iterative introspection for meta-review gen-
eration with prompting (Zeng et al., 2024), our
work is based on a three-layer sentiment consoli-
dation framework and focuses on various review
facets, and we explicitly investigate the sentiment
fusion process which is arguably an important as-
pect of meta-review generation.


2 Related Work

Over the past few years, several studies have been
accomplished on meta-review generation. Some re-
searchers have employed rule-based techniques in
conjunction with deep neural network architectures
(Bhatia et al., 2020; Pradhan et al., 2021), while
others proposed encoder-decoder-based methods
(Kumar et al., 2021; Li et al., 2023)to tackle the
meta-review generation task. Recent developments
with Large Language Models (LLMs), including
but not limited to GPT-3.5 and GPT-4 (Brown
et al., 2020; Ouyang et al., 2022), PaLM (Thop-
pilan et al., 2022), LLaMA (Touvron et al., 2023a),
Bloom (Scao et al., 2022), GLaM (Du et al., 2022),
have shown remarkable performance in traditional
summarization tasks. Yet, their performance on
complex, i.e., multi-constraint multi-document
summarization tasks (Bansal et al., 2022b)like
meta-review composition is still understudied.
Recently, Du et al. (2024)examined the effective-
ness of large language models (LLMs) in both re-
viewing and meta-reviewing research papers. Sim-
ilarly, Tyser et al. (2024)evaluated LLMs’ ability
to review papers and compared their quality with
human-written peer reviews. In another line of
work, Zeng et al. (2024)introduced a Checklist-
guided Iterative Introspection (CGI2) approach
using LLMs, which breaks down scientific opin-
ion summarization into several stages. However,
LLMs are quite sensitive to prompts that are fed
to them (Loya et al., 2023; Sclar et al., 2023), and
therefore, designing appropriate prompts with the
right amount of detail has become more important
than ever (Liu et al., 2023a; Han et al., 2022). This
issue worsens in practice as there is no standard
taxonomy of prompts to follow for benchmarking
LLMs on complex tasks that the community has a
general consensus on yet. As such, the main mo-
tivation of this work, which makes our case study
more compelling, stems from the following two
gaps in the literature: 1) LLM’s performance on
multi-constraint multi-perspective summarization
tasks (e.g., meta-review composition) is still under-
studied, 2) no study has yet followed a standard
prompting taxonomy to systematically compare
LLMs on such complex tasks.
Fortunately, very recently, Santu and Feng
(2023)have proposed a general prompting taxon-
omy called TELeR, which can serve as a unified
standard for comparing and benchmarking LLMs’
performances on complex generation tasks (de-
7765
tails in appendix). In this work, we leveraged
this TELeR taxonomy for designing prompts in
the context of a meta-review composition task. We
reported the specific categories of prompts we ex-
perimented with across multiple LLMs. This en-
abled more meaningful comparisons among the
three LLMs we studied and, thereby, helped to de-
rive more accurate conclusions about their relative
performances.


2 Related Work

2.1 Opinion Summarization
The task of opinion summarization is typically decomposed
into three stages: aspect extraction, which identifies the spe-
cific features discussed in reviews; polarity identification,
which assesses whether the sentiment towards each aspect
is positive, negative, or neutral; and summary generation,
which compiles these aspects and sentiments into a cohesive
summary of the opinions [Hu and Liu, 2006].The lack of
parallel data in review summaries limits most methodologies
into the few-shot abstractive setting [Brazinskas et al.,2020a;
Brazinskas et al.,2022],or unsupervised extractive set-
ting [Angelidis and Lapata, 2018; Angelidis et al.,2020;
Chowdhury et al.,2022] where the aspects and sentiments
from the input reviews are collected, selected, and rearranged
into the output meta-reviews.
Only a few previous opinion summarization
datasets [Wang and Ling, 2016] contain gold-standard
summaries and support supervised training of abstractive
models [Amplayo and Lapata, 2019].Pretrained aspect-
based sentiment analysis [Suhara et al.,2020],variational
autoencoders [Brazinskas et al.,2020b; Chu and Liu, 2019;
Iso et al.,2021; Isonuma et al.,2021] and large language
models [Bhaskar et al.,2022] enable unsupervised ab-
stractive approaches, where the generated summaries are
validated to be more fluent, informative, coherent, and
concise compared to traditional extractive summaries.
To support the training and evaluation of supervised meth-
ods, recent work constructs synthetic datasets by random
sampling [Shen et al.,2023],adding noise to the sam-
pled summary to generate documents [Amplayo and Lapata,
2020],searching for relevant reviews to act as the input docu-
ment set [Elsahar et al.,2021],or sampling with trained mod-
els [Amplayo et al.,2021a; Amplayo et al.,2021b].However,
synthetic pseudo-summaries in the product review domain are
known to be detached from real-world distributions, be pos-
sibly irrelevant or inconsistent with input documents, and are
known to ignore important underlying details.
2.2 Meta-review Generation
The first attempt to generate paper meta-reviews is Meta-
Gen [Bhatia et al.,2020],which generates an extractive sum-
mary draft then uses a fine-tuned model for decision predic-
tion and abstractive review generation. [Kumar et al.,2021]
emphasizes decision awareness, proposing a model for deci-
sion prediction and subsequent meta-review generation. The
most similar work to ours is MReD [Shen et al.,2022],where
7,089 paper meta-reviews from ICLR 2018 - 2021 are man-
ually annotated with sentence-level structure labels. These
structure labels categorize sentences based on their function
in the document, such as summary, evaluation, or recom-
mendation. The difference between their work and ours is
that they focus on structure-controlled text generation, while
our work 1) enables scientific opinion summarization with a
larger corpus, 2) provides a prompting-based solution, and
3) performs broader evaluations. Note that while there are
other concurrent efforts to collect paper meta-reviews or re-
views [Dycke et al.,2023],we are the first to model meta-
review generation as scientific opinion summarization and to
offer a unified dataset covering a broad range of conference
venues.
